GRaCE: Balancing Multiple Criteria to Achieve Stable, Collision-Free, and Functional Grasps

This paper addresses the multi-faceted problem of robot grasping, where multiple criteria may conflict and differ in importance. We introduce a probabilistic framework, Grasp Ranking and Criteria Evaluation (GRaCE), which employs hierarchical rule-based logic and a rank-preserving utility function for grasps based on various criteria such as stability, kinematic constraints, and goal-oriented functionalities. GRaCE's probabilistic nature means the framework handles uncertainty in a principled manner, i.e., the method is able to leverage the probability that a given criteria is satisfied. Additionally, we propose GRaCE-OPT, a hybrid optimization strategy that combines gradient-based and gradient-free methods to effectively navigate the complex, non-convex utility function. Experimental results in both simulated and real-world scenarios show that GRaCE requires fewer samples to achieve comparable or superior performance relative to existing methods. The modular architecture of GRaCE allows for easy customization and adaptation to specific application needs.

==> content/rebuttal.tex <==
\section*{General Response}

We thank the Area Chair (\ac{}) and reviewers (\rone{} [e955], \rtwo{} [iRVC], \rthree{} [X9K2]) for your positive comments about \method{} and  your constructive feedback. We have incorporated your comments into our revision. Edits to the manuscript are shown in \rev{blue}. Specifically, we have revised the paper to clarify the benefits of \method{} and added results from the suggested ablation experiments. Please see detailed responses to individual reviewers below. 


\section*{Specific Responses to \rone{} [e955]}

\para{Ablation on performance with just gradient-based optimization or gradient-free optimization.} Thank you for this suggestion. We have conducted this ablation on the Shelf environment and added the results to the paper (Sec. \ref{sec:ablations}). Briefly, using either solely gradient-based or gradient-free optimization leads to far poorer results, as shown in the figure below. We have added this ablation experiment to the paper. 
\begin{center}
\includegraphics[width=0.8\linewidth]{content/figs/grad_vs_nongrad.pdf}
\end{center}

\para{Selection of and sensitivity to hyperparameters.} We selected our hyperparameters based on available computational resources. We have added additional details and experiments to the paper (Sec. \ref{sec:ablations}): briefly, increasing $T$ and $K$ improves success rates, with the cost of added computation time. For example, the figure below shows increases in both performance and optimization time with varying $T$ but fixed $K=2$.
\begin{center}
\includegraphics[width=0.8\linewidth]{content/figs/T_ablation.pdf}
\end{center}

\para{Only calculating the gradients for the most expensive criterion.} This is an interesting idea. Of the three, The Stability classifier was the most computationally expensive since it requires backpropagation through the network that contains several layers of MLP, CNN and PointNet++. We tried your suggestion to only compute the gradient of Stability classifier at intervals; this reduced computation costs by 15\% but reduced the number of successful grasp by 50\%. Future work can go into improving the optimization routine, but we also note that we currently use an un-optimized stability classifier written in Python. We believe computation time can be significantly reduced by using \method-OPT with a more efficient model. 

\section*{Specific Responses to \rtwo{} [iRVC]}

\para{How changes in ranking affect outcomes.} Thank you for pointing this out. As suggested, we have run an additional ablation experiment to examine the effect of how changing the priorities can affect the results. We ran the same experiment on the Shelf environment, but changed the priorities of the Execution (E) and the Collision (C) classifiers. 

The table below shows the average scores of the grasps on each of the different criteria. Compared to the initial sampled grasps, \method{} improves scores differently depending on the specified ranks. For example, when C was prioritized over E (S$>$C$>$E), the average score for the collision criteria was 0.89. This fell to 0.63 when the E classifier had a higher priority (S$>$E$>$C). The score for the Stability criteria remained relatively unchanged since its priority wasn't altered. We hope this illustrates how different priority specifications alters the obtained grasps. We have revised the paper with this experiment.

\begin{center}
\begin{tabular}{lccc}
\hline
                           & S        & E        & C        \\ \hline
Initial                         & 0.26 & 0.57 & 0.30 \\ \hline
S\textgreater{}C=E              & 0.70 & 0.63  & 0.83 \\
S\textgreater{}C\textgreater{}E & 0.69 & 0.56  & 0.89 \\
S\textgreater{}E\textgreater{}C & 0.72 & 0.76   & 0.63 \\
\hline
\end{tabular}
\end{center}

\para{Clarification on the benefits of the probabilistic approach.} The main benefit of \method{} is to handle \emph{uncertainty} in a principled manner. Uncertainty is prevalent in real robot settings (e.g., due to partial observability or noise) and unlike Veer et al, \method{}'s probabilistic setup enables us to incorporate the probability that a criterion is satisfied and the \emph{expected} ranks of grasps. We agree this point was initially unclear and have edited the introduction to clarify this benefit.

\para{Minor errors.} We have revised the manuscript to correct the missing definition of $\sigma$ (it is the logistic sigmoid function). We have also modified the diagram in Fig 4 to better illustrate the computational advantages of \method{}.


\section*{Specific Responses to \rthree{} [X9K2]}

\para{Failure sources for real-world experiments.} We have revised the paper with the following table that breaks down the different failure types as percentages. We recorded three kinds of failures: (i) Robot Errors (RE) where the robot fails to plan to the target grasp or stops due to a singularity, (ii) Grasp Failure (GF) refers to cases where the robot collides with an object or the environment, or grasps nothing, and (iii) No Grasp (NG) occurs when no sufficiently good grasp was generated (all expected utilities were below $0.01$). 
\begin{center}
{\small
\begin{tabular}{l|ll|ll}
\hline
              & \multicolumn{2}{c|}{Box}                      & \multicolumn{2}{c}{Bowl}   \\ \hline
              & Filter                          & GRaCE       & Filter      & GRaCE        \\ \hline
RE   & \multicolumn{1}{r}{16\% (0.03)} & 31\% (0.03) & 12\% (0.06) & 20\% (0.014) \\
GF & 58\% (0.12)                     & 69\% (0.08) & 50\% (0.1)  & 30\% (0.07)  \\
NG      & 26\% (0.12)                     & 0\% (0.00)  & 38\% (0.06) & 50\% (0.07) \\ \hline
\end{tabular}
}
\end{center}


% \para{multiple IK solutions may exist, how is theta chosen?} Tas fill this in. 

\para{Clarification on IK and $\mathbf{\theta}$.} We use IKNet~\cite{bensadoun2022neural}, a state-of-the-art differentiable inverse kinematic solver. Given the initial guess and target pose, IKNet outputs the inverse kinematics ($\mathbf{\theta}$ for our E classifier). It also handles multiple solutions for redundant robots, in which the inverse kinematic solution is the pose closest to the initial guess in SE(3). Since the IK solver is imperfect, we check if the pose is within tolerance, $d_{\epsilon}$, of the solver as shown in Eq.~\ref{eq:execution_classifier}. If no inverse kinematics solution exists for the pose, it returns the closest robot configuration (projected pose onto the robot's workspace) to the initial guess. In this case, the $\mathbf{g}$ and $\tilde{\mathbf{g}}$ are not the same. Thus, we calculate the distance between the grasp and the projected grasp onto the robot's workspace for E classifier as specified in Eq.~\ref{eq:execution_classifier}. 

\para{Choice of sample-and-filter threshold.} For the  S and E classifiers, the thresholds are set to be  0.9999. For the S classifier, we set it as 0.9 which gave us good results in preliminary trials.

\para{Lack in clarity as to what GRACE alone would be.} We agree and have clarified this in the revision. \method{} is a \emph{probabilistic grasp ranking framework} that leads to the expected utility function in Eq (2). This utility can be maximized in various ways and in this work, we introduce \method-OPT, which blends gradient-free and gradient-based optimized. 

\para{Missing supplementary material.} This was a typo in the paper: we have corrected it to specify ``online code repository''; we plan to release source code to reproduce our experiments. 

\para{JointBERT model and classifier contexts.} For the JointBERT model, we curated the dataset ourselves but do not claim this as a contribution. The point cloud is indeed the context to the stability and collision criteria. The context for the execution criterion is the robot configuration.  

\para{Minor comments/suggestions.} Thank you for the detailed recommendations. We have incorporated your suggestions to improve the captions in Figs 5, 6, and 8. Thank you for the suggestion to remove Table I and II; both were inserted as some of our proof-readers found our method too abstract and wanted a better handle on how the different elements (e.g., priority, rule, rank) fit together. We will leave the Tables in for now and hope you understand our decision. We also commit to expanding the literature around task-oriented grasping.

%Thank you again for your effort in reviewing our paper and we believe the revision is much improved thanks to your constructive feedback! 

% The point cloud is an input to the S and C classifiers, while the input to the E classifier is robot configuration.



% \textbf{In training the JointBERT model, was the curated dataset from a previous method or was that generated as part of the contribution of this paper?}
% The curated dataset used to train the JointBERT model was programmatically generated from a set of common objects and actions, for a total of 9164 variations of user intents, e.g. ``grasp the box to the right of the scissor''. 

% \textbf{context to the probability of the criteria satisfaction the point cloud?} 




\section*{Summary Response to AC and Reviewers}

Thank you again to the AC and reviewers for your helpful feedback. We believe our paper has improved thanks to your comments and I hope we have addressed your concerns. If so, we hope you will consider accepting our paper for publication.
